Improving Performance of Iterative Methods by Lossy Checkponting

Iterative methods are commonly used approaches to solve large, sparse linear systems, which are fundamental operations for many modern scientific simulations. When the large-scale iterative methods are running with a large number of ranks in parallel, they have to checkpoint the dynamic variables periodically in case of unavoidable fail-stop errors, requiring fast I/O systems and large storage space. To this end, significantly reducing the checkpointing overhead is critical to improving the overall performance of iterative methods. Our contribution is fourfold. (1) We propose a novel lossy checkpointing scheme that can significantly improve the checkpointing performance of iterative methods by leveraging lossy compressors. (2) We formulate a lossy checkpointing performance model and derive theoretically an upper bound for the extra number of iterations caused by the distortion of data in lossy checkpoints, in order to guarantee the performance improvement under the lossy checkpointing scheme. (3) We analyze the impact of lossy checkpointing (i.e., extra number of iterations caused by lossy checkpointing files) for multiple types of iterative methods. (4)We evaluate the lossy checkpointing scheme with optimal checkpointing intervals on a high-performance computing environment with 2,048 cores, using a well-known scientific computation package PETSc and a state-of-the-art checkpoint/restart toolkit. Experiments show that our optimized lossy checkpointing scheme can significantly reduce the fault tolerance overhead for iterative methods by 23%~70% compared with traditional checkpointing and 20%~58% compared with lossless-compressed checkpointing, in the presence of system failures.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> tex/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

In this section, we first discuss the importance of checkpointing for iterative methods on HPC environments. Then, we discuss how to integrate our lossy checkpointing with existing HPC applications. Finally, we discuss the impact of our lossy checkpointing on the reproducibility of iterative methods and outer applications. \vspace{-1mm}

\paragraph{Importance of Checkpointing for Iterative Methods}
Iterative methods for solving sparse linear systems are one of the most crucial components determining the scalability and efficiency of HPC applications. Becciani et al. \cite{becciani2014solving} presented a study of solving very large-scale sparse linear systems (up to 72 billion linear  equations and 600 million unknowns) with an ad-hoc implementation of the iterative solver---preconditioned Sparse Equations and Least Squares (PC-LSQR) \cite{pc-lsqr}---on a IBM BlueGeneQ system using both MPI and OpenMP. These sparse linear systems are arise from a 5-parameter astrometric catalogue at the micro-arcsecond level for about 1 billion stars of our Galaxy under a cornerstone mission (called Gaia) launched by European Space Agency. Their experimental results show that solving a very large-scale sparse linear system with $7.2\times 10^{10}$ equations for the last period of the Gaia mission needs to take about 1,000 to 4,000 iterations for convergence (49 seconds per iteration), totally up to $1.96\times 10^{5}$ seconds (i.e., more than 54 hours), using 2,048 BlueGeneQ nodes (each node equipped with 16 processor cores and 16 GB of SDRAM memory).

We also evaluate the productive execution time of GMRES with the largest symmetric indefinite sparse matrix (i.e., KKT240 with around 28 million linear equations) in the University of Florida Sparse Matrix Collection \cite{ufl} using 4,096 processes/cores on the Bebeop cluster at Argonne, as shown in Figure \ref{fig:f10}. Symmetric indefinite KKT matrices are generated from a nonlinear programming problems for a 3D PDE-constrained optimization problem \cite{nlpkkt}. We refer readers to \cite{nlpkkt240} for more details of the matrices. Note that we use GMRES for demonstration purpose, since it is much faster than Jacobi and CG cannot handle indefinite matrix. We test all the preconditioners listed in the PETSc's website \cite{petsc-linear-solver} and choose the best one (i.e., Jacobi preconditioner). We use the relative convergence tolerance of $1\mathrm{e}{-6}$. Figure \ref{fig:f10} shows that the average productive execution time for solving KKT240 once with GMRES needs to take more than one hour with 4,096 processes. Moreover, we note that the dimensions of the matrices collected by UFL Sparse Matrix Collection grow exponentially with years \cite{ufl}. 

\begin{figure}[]
\centering
\includegraphics[scale=0.50]{Fig/Fig10.pdf}
\vspace{-3mm}
\caption{Average productive execution times and numbers of convergence iterations for solving KKT240 once using GMRES and Jacobi preconditioner with different number of processes on Bebop.}
\label{fig:f10}
\vspace{-3mm}
\end{figure}

Therefore, on one hand, it will be more common to spend hours to days running iterative methods with a large number of ranks in parallel for very large-scale sparse linear systems; on the other hand, the mean time between failures for petascale supercomputers could be hourly or even less than one hour, as demonstrated by a recent study \cite{liu2018large} based on a three-year statistic of Sunway TaihuLight supercomputer \cite{fu2016sunway}. Taking these two factors into account, we believe that checkpointing during iterative methods is very important for the future HPC applications and exascale systems. \vspace{-1mm}

\paragraph{Integration of Lossy Checkpointing}
Users can follow the below workflow to easily integrate our lossy checkpointing for linear iterative solver with existing HPC applications: (1) initialize application; (2) \textit{register variables external to the solver to checkpoint}; (3) start application's computations/iterations; (4) enter the solver's library; (5) \textit{register the solver's variables to checkpoint in the library}; (6) iterate the solver; (7) \textit{save or restore the application and solver's variables}; (8) continue to iterate the solver; (9) exit the solver's library; (10) continue application's computations/iterations (if needed); (11) exit application. Specifically, users can use the APIs, \texttt{Protect()} and \texttt{Snapshot()}, provided by our lossy checkpointing library to register and save/restore variables, as discussed in (2), (5), and (7). \vspace{-1mm} 

%Application developer only needs to register the necessary dynamic vectors (such as solution and residual vector) in lossy mode and the dynamic state variables (such as number of iterations) in lossless mode outside of the library and checkpoint them along with the iterations. Our design principle is the same as that of existing state-of-the-art checkpointing libraries, such as FTI \cite{fti} and SCR \cite{scr}, that is to separate the responsibility between application developer and checkpointing library developer. \vspace{-1mm}

\paragraph{Reproducibility with Lossy Checkpointing}

Based on our experiments, iterative methods with our lossy checkpointing can still converge to a solution that satisfies the user-set accuracy. Moreover, the variance of the solution is much smaller than the user-set convergence tolerance threshold. Hence, our lossy checkpointing has an impact on bit-level reproducibility but only has a negligible impact on tolerance-based reproducibility of iterative methods and outer applications. %\vspace{-1mm}
%Our lossy checkpointing only produces a machine accuracy level variance to the converged solution based on our experiments. Hence, our lossy checkpointing only has an impact on bit-level rather than tolerance-based reproducibility of the iterative methods and outer applications.
